Byzantine Consensus in Abstract MAC Layer

This paper studies the design of Byzantine consensus algorithms in an \textit{asynchronous }single-hop network equipped with the "abstract MAC layer" [DISC09], which captures core properties of modern wireless MAC protocols. Newport [PODC14], Newport and Robinson [DISC18], and Tseng and Zhang [PODC22] study crash-tolerant consensus in the model. In our setting, a Byzantine faulty node may behave arbitrarily, but it cannot break the guarantees provided by the underlying abstract MAC layer. To our knowledge, we are the first to study Byzantine faults in this model. We harness the power of the abstract MAC layer to develop a Byzantine approximate consensus algorithm and a Byzantine randomized binary consensus algorithm. Both of our algorithms require \textit{only} the knowledge of the upper bound on the number of faulty nodes $f$, and do \textit{not} require the knowledge of the number of nodes $n$. This demonstrates the "power" of the abstract MAC layer, as consensus algorithms in traditional message-passing models require the knowledge of \textit{both} $n$ and $f$. Additionally, we show that it is necessary to know $f$ in order to reach consensus. Hence, from this perspective, our algorithms require the minimal knowledge. The lack of knowledge of $n$ brings the challenge of identifying a quorum explicitly, which is a common technique in traditional message-passing algorithms. A key technical novelty of our algorithms is to identify "implicit quorums" which have the necessary information for reaching consensus. The quorums are implicit because nodes do not know the identity of the quorums -- such notion is only used in the analysis.

==> impossibilityIntuition.tex <==
\section{Without the Knowledge of $f$, it is Impossible to Solve Consensus}

In this section, we provide the intuition for our proof that without the knowledge of $f$, it is impossible to solve consensus. The full proof is included in Appendix \ref{app:impossible}.

We construct an indistinguishably proof by constructing scenarios in which there is no way for a node $i$ to distinguish whether another node $j$’s behavior is Byzantine or not, which could lead to a violation of validity. We assume the existence of an algorithm $A$ which solves consensus for a certain $n$ and $f$ without the knowledge of these values. We construct two scenarios with different value for $n$ and $f$. These scenarios remain indistinguishable to all nodes because no nodes have knowledge of $n$ or $f$. In the first scenario, node $i$ can only communicate with one other node to update its state, and in the second, node $i$ can receive messages from $\geq 2f+1$ other nodes within the system. In the second scenario, we impose a time delay, $D$, on all messages sent from any node other than an arbitrary node $j$. We observe that within the time interval $(0, D]$, a node $i$ cannot distinguish between the two scenarios (whether there is only one, or more than one other nodes within the system). Now, node $i$ has no way of determining whether the behavior of node $j$ is Byzantine or fault-free. Node $i$ then runs algorithm $A$, and may output a value that is outside the range of fault-free inputs if $i$ considers a Byzantine node $j$’s value, hence, violating validity.

==> lowerBound.tex <==
\section{Impossibilities}
\label{app:impossible}

% \subsection{System Parameter requirements}
% In this section, we provide proofs for two system parameters which always hold. Firstly, we prove that if the total number of nodes within the system is less than double the number of Byzantine nodes, then it is not possible to define an algorithm which solves consensus within the system. Secondly, we also prove that without the knowledge of the number of Byzantine nodes within the system, it is impossible to solve consensus.

% \subsection{Proof that NO algorithm exists if $n \leq 2f$}

% \begin{theorem}
%     NO algorithm exists if $n \leq 2f$.
% \end{theorem}

% \begin{proof}

% Consider the case that $n \leq 2f$. 
    
%     Scenario 1: Let both node $a$ and node $b$ be correct nodes.
    
%     Suppose node $a$ has input $0$ and node $b$ has input $1$.
    
%     To satisfy validity, there must be an output which can be any value in the range $[0, 1]$ at $a$ and $b$ such that $\epsilon$-agreement is satisfied. In fact, $a$ can have one value and $b$ can have one value as long as $|a - b| \leq \epsilon$.
    
%     Consider the cases (i) and (ii) below following from Scenario 1:
    
%     (i) $b$ outputs 1 in Scenario 1: 
    
%     Now consider Scenario 3. Assume the Byzantine node $b$ behaves in the exact same manner as it did in Scenario 1 to node $a$ (note that we are now considering a Byzantine $b$). From the perspective of node $a$, Scenario 1 and Scenario 3 are indistinguishable - there is no way for node $a$ to know whether the behavior from $b$ is Byzantine or not. Therefore, node $a$ outputs $[1-\epsilon, 1]$, but this is a contradiction because any value in $[1-\epsilon, 1]$ is not within the range of fault-free inputs, $[0]$, so it violates validity.
    
%     (ii) $b$ outputs a value in $[0, 1)$ in Scenario 1: 
    
%     Now consider Scenario 2. Assume the Byzantine node $a$ behaves in the exact same manner as it did in Scenario 1 to node $b$ (note that we are now considering a Byzantine $a$). From the perspective of node $b$, Scenario 1 and Scenario 2 are indistinguishable - there is no way for node $b$ to know whether the behavior from $a$ is Byzantine or not. Therefore, node $b$ outputs $[0, 1)$, but this is a contradiction because any value in $[0, 1)$ is not within the range of fault-free inputs, $[1]$, so it violates validity.
    
% \end{proof}

\subsection{Proof that without the knowledge of $f,$ it is impossible to solve consensus}

\begin{theorem}
    Without the knowledge of $f,$ it is impossible to solve consensus.   
\end{theorem}

\begin{proof}
    Assume that there exists a uniform algorithm $A$ that solves consensus for a certain $n$ and $f$, but the algorithm itself does not know these values for $n$ and $f$. An algorithm is uniform is all nodes are using the same algorithm. 
    
    To satisfy $\epsilon$-agreement, all $n-f$ fault-free nodes must have an output such that no two fault-free noes $i$ and $j$ have states $|v_i - v_j| > \epsilon$.
    
    Consider Scenario 1 and Scenario 2 below. In both scenarios, the nodes do not know the exact value of $n$, nor $f$:
    
    1. Scenario 1: Suppose $n = 2$, $f = 0$. Assume two nodes, $a$ and $b$, are fault-free nodes. A node can only communicate with one other node to make a decision, since $n=2$. 
    
    Suppose node $a$ has input $0$ and node $b$ has input $1$.
    
    To satisfy validity, there must be an output which can be any value in the range $[0, 1]$ at $a$ and $b$ such that $\epsilon$-agreement is satisfied. In fact, $a$ can have one value and $b$ can have one value as long as $|v_a - v_b| \leq \epsilon$.
    
    2. Scenario 2: Assume there are any number of nodes within the system satisfying $n \geq 2f + 1$. In this scenario, a node, say node $a$, can only communicate with one other node to make a decision. This is because to node $a$, it is indistinguishable whether $a$ is in Scenario 1 or Scenario 2 since there is no way for node $a$ to know the values of $n$ or $f$. 
    
    We can impose a delay $D$ on all messages other than those from node $b$. 
    
    Similar to the setup in [Churn paper], assume that $D$ is an unknown upper bound, on the delay of any message sent between between fault-free nodes. Let $D = t' - t$ where $D > 0$ be the maximum delay on a message sent at time $t$ and received at time $t'$.
    
    For two fault-free nodes $a$ and $b$, if a message sent from node $a$ at time $t$ and node $b$ is active throughout $[t, t + D]$, then we know that node $b$ will receive the message from $a$, and that the delay of every received message is in the range $(0, D]$.
    
    Assume $(0, D]$ is the bound on the delay of the message sent from node $b$. In the time interval $(0, D]$, assume the only message which node $a$ receives is a message from node $b$. During this time interval, node $a$ cannot distinguish between Scenarios 1 and 2.
    
    Run $A$ in Scenario 2, within the time interval $(0, D]$, assuming the Byzantine node $b$ behaves in the exact same manner as it did in Scenario 1 to node $a$. Once again, from the perspective of node $a$, Scenarios 1 and 2 remain indistinguishable and there is no way for node $a$ to know whether the behavior from $b$ is Byzantine or not. Node $a$ can output a value in $(0, 1]$, but this is a contradiction because any value in $(0, 1]$ is not within the range of fault-free inputs, $[0]$, so validity is violated.    
    
    Next, run $A$ in Scenario 2, this time assuming the Byzantine node $a$ behaves in the exact same manner as it did in Scenario 1 to node $b$. Once again, from the perspective of node $b$, Scenarios 1 and 2 remain indistinguishable and there is no way for node $b$ to know whether the behavior from $a$ is Byzantine or not. Node $b$ can output a value in $[0, 1)$, but this is a contradiction because any value in $[0, 1)$ is not within the range of fault-free inputs, $[1]$, so validity is violated. 
\end{proof}



==> random-3f+1.tex <==
\newpage
\section{Byzantine Random Consensus without Knowledge of $n$}

\subsection{System Model}
We adopt the same system model as defined in Section 3.1, with the modification that $n \geq 3f + 1$.

\begin{definition}[Condition WAIT]
    In phase $p$, node $i$ satisfies Condition WAIT with value $v$, if there exist two sets of nodes $X$ and $Y$ such that

    \begin{enumerate}
    
        \item $|X| \geq 2f+1$;
        
        \item $i$ received $(COMPLETE_{EV}, p_i)$ message for each $x\in X$;

        \item $i$ received $(AUX, v, p)$ message for each $x\in X$; 
        
        \item $|Y| = |U_i|-f$;
        
        \item $i$ received $(AUX, *, p)$ message for each $y\in Y$;
        
        \item $X \subseteq Y$;
        
        \item $value_i[p]$ is the set of values received from $Y$'s $(AUX, *, p)$ messages; 
        
        \item $value_i[p] \subseteq estValues_i[p]$.
        
    \end{enumerate}
\end{definition}

~

\begin{comment}
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}
\begin{algorithm}
\caption{BV-broadcast}
\label{alg:simple-RBC}
\begin{algorithmic}[1]
\footnotesize
    \item[] \textbf{operation} BV-broadcast$(v_i, p_i)$ \textbf{is}
    \INDSTATE[] \textbf{mac-broadcast}(B-val($EST, v_i$))
    \\\hfill
    \item[] \textbf{when} B-val($EST, v$) \textbf{is received} 
    \IF{B-val($EST, v$) is received from $f + 1$ nodes and B-val($EST, v$) not yet broadcast}
        \STATE \textbf{mac-broadcast}(B-val($EST, v$))
    \ENDIF
    \IF{B-val($EST, v$) is received from $2f + 1$ nodes}
        \STATE $estValues_i[p_i] \gets estValues_i[p_i] \cup \{v\}$
    \ENDIF
\end{algorithmic}
\end{algorithm}
\end{comment}
~

\begin{algorithm}
\caption{Simple RBC: Steps at each node $i$}
\label{alg:simple-RBC}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:}]
    
    \item[] $p_i$ \COMMENT{phase, initialized to $0$}
    
    \item[] $v_i$ \COMMENT{state, initialized to $x_i$, the input at node $i$} 

    \item[] $U_i$ \COMMENT{count, initialized to $\{\}$, set of all the nodes that node $i$ knows so far} 
    
    %\item[] $R_i[p] \leftarrow \{\}$ \COMMENT{set of received phase-$p$ messages}
    
    \item[] \hrulefill
    \begin{multicols}{2}    

    \WHILE{true}
        \STATE $p_i \gets p_i+1$

        \STATE \textbf{mac-broadcast}$(EST, v_i, p_i)$

        \STATE \textbf{wait until} $estValues_i[p_i] \neq \emptyset$ and $i$ has received $ACK$ from mac-broadcast on Line 25

        %\FOR{each $w \in estValues_i[p_i]$}
        %    \STATE \textbf{mac-broadcast}$(AUX, w, p_i)$
        %\ENDFOR
        
        \STATE \textbf{mac-broadcast}$(EST\_VALS, estValues, p_i)$
        \STATE \textbf{mac-broadcast}$(COMPLETE\_EV, p_i)$
 
        \STATE \textbf{wait until} Condition WAIT is satisfied \\\hspace{20pt}with some value $z$
        
        %$\exists$ a set of $2f+1$ $(COMPLETE, -)$ messages such that $values_i[p_i] \subseteq estValues_i[p_i]$ where $values_i[p_i]$ is the set of values carried by some $|U_i|-f$ $AUX$ messages 


        \STATE $c \gets coinflip()$

        \IF{$values_i[p_i] = \{v\}$}
            \IF{$v = c$}
                \STATE output $v$
            \ENDIF
            \STATE $v_i \gets v$
        \ELSE
            \STATE $v_i \gets c$     
        \ENDIF
    \ENDWHILE

    \columnbreak
    \item[//\textit{Background AUX message handler}]
    \item[\textbf{Upon} receiving $(AUX, v_j)$ \textbf{do}]
    \STATE $U_i \gets U_i \cup \{j\}$
    \\\hfill

    \item[//\textit{Background EST message handler}]
    \item[\textbf{Upon} receiving ($EST, v, p$) \textbf{do}] 
    \IF{($EST, v, p$) is received from $f + 1$ nodes and ($EST, v, p$)) not yet broadcast by $i$}
        \STATE \textbf{mac-broadcast}($EST, v, p$))
    \ENDIF
    \IF{($EST, v, p$) is received from $2f + 1$ nodes}
        \STATE $estValues_i[p] \gets estValues_i[p] \cup \{v\}$
        \STATE \textbf{mac-broadcast}$(AUX, w, p_i)$
        \STATE \textbf{mac-broadcast}$(COMPLETE, estValues_i, p_i)$
    \ENDIF
\end{multicols}  
\end{algorithmic}
\end{algorithm}


 
    
    


==> random.tex <==
\section{Byzantine Random Consensus without Knowledge of $n$}

\begin{algorithm}
\caption{Simple RBC: Steps at each node $i$}
\label{alg:simple-RBC}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:}]
    
    \item[] $p_i$ \COMMENT{phase, initialized to $0$}
    
    \item[] $v_i$ \COMMENT{state, initialized to $x_i$, the input at node $i$} 

    \item[] $U_i$ \COMMENT{count, initialized to $\{\}$, set of all the nodes that node $i$ knows so far} 
    
    %\item[] $R_i[p] \leftarrow \{\}$ \COMMENT{set of received phase-$p$ messages}
    
    \item[] \hrulefill
    \begin{multicols}{2}    

    \WHILE{true}
        \STATE $p_i \gets p_i+1$
        \STATE \textbf{mac-broadcast}$(AUX, v_i)$

        \STATE \textbf{mac-broadcast}$(complete, i)$
 
        \STATE \textbf{wait until} $\exists$ a set of $2f+1$ $(complete, -)$ messages such that $values_i \subseteq bin\_values_i[r_i]$ where $values_i$ is the set of values carried by any $|U_i|-f$ messages 

        \STATE $R_i[p_i] \gets$ $v$ field in all received $values_i$ messages \COMMENT{$R_i$ is a multi-set}

        \STATE $C_i[p_i] \gets$ any value $v$ that appears at least $f+1$ times in $R_i[p_i]$

        \STATE $c \gets coinflip()$

        \IF{$C_i[p_i] = \{v\}$}
            \IF{$v = c$}
                \STATE output $v$
            \ENDIF
            \STATE $v_i \gets v$
        \ELSE
            \STATE $v_i \gets c$     
        \ENDIF
    \ENDWHILE

    \columnbreak
    \STATE //\textit{Background message handler}
    \STATE \textbf{Upon} receive $(AUX, v_j)$ do
    \STATE $U_i \gets U_i \cup \{j\}$
\end{multicols}  
\end{algorithmic}
\end{algorithm}

% Logic of keeping track of value_i
    
On Line 3, each node $i$ sends a mac-broadcast$(AUX, v_i)$. To proceed to Line 4, node $i$ must receive the MAC-ACK from the Line 3 mac-broadcast. 

On Line 4, each node $i$ sends a mac-broadcast$(complete, i)$ signifying that node $i$ has received its MAC-ACK from Line 3. 

Each node $i$ then waits at Line 5 until the condition that there exists a set of $2f+1$ $(complete, -)$ messages such that $values_i \subseteq bin\_values_i[r_i]$ where $values_i$ is the set of values carried by any $|U_i|-f$ messages. $bin\_values_i[r_i]$ is the local set of fault-free values received by node $i$. Line 5 defines $values_i$ as the set of values broadcast on Line 3 by $|U_i| - f$ different nodes. $values_i$ contains at least $|values_i| - f$ fault-free values from the set $U_i$ which node $i$ has received from the $|U_i|$ other nodes it has identified within the system. Therefore, after Line 5, $values_i \in \{0, 1\}$.

At Line 6, $R_i$ is assigned to be the multiset of the $v$ field in all received $values_i$ messages. $R_i$ contains at least $2f + 1$ of the values from the $|U_i|$ $(AUX, v)$ messages sent on Line 3.

Line 7 ensures that any values added to $C_i[p_i]$ must be within the range of fault-free values. If $v$ appears at least $f + 1$ times, since there are at most $f$ Byzantine nodes, at least one of these occurrences must have been sent by a fault-free node.

At line 8, each node $i$ sets the local variable $c$ to be the value of the common coin corresponding to the current round.

Line 9 determined the size of $C_i[p_i]$. If $C_i[p_i] = \{v\}$, $|C_i[p_i]| = 1$, there is only one value in $values_i$ within the fault-free range. If $c = v$, node $i$ outputs $v$. Otherwise, if $c \neq v$, node $i$ updates its state $v_i$ to take the value $c$ in the subsequent round. If $|C_i[p_i]| = 2$, then we know that $C_i[p_i] = \{0, 1\}$, meaning that both $0$ and $1$ have been sent/ received by fault-free nodes. In this event, node $i$ updates its state $v_i$ to take the value $c$ in the subsequent round.


\begin{lemma}
    Fix a phase $p$. For any fault-free $i$ and $j$ with $C_i[p] = \{v\}$ and $C_j[p] = \{u\}$, then $v = u$.
\end{lemma}

\begin{proof}
    Assume node $i$ completes Line 5 at time $T_i$. Without loss of generality, assume node $j$ completes Line 5 at or after $T_i$. Let $A_i$ be the set of nodes from which $i$ receives $(complete, -)$ messages. Now, we can make the following observation:

    \begin{itemize}
        \item $A_i$ must contain at least $f+1$ fault-free nodes which has completed Line 4 with value $v$ before $T_i$. This is because these nodes have already started Line 5. And, in order for node $i$ to have completed Line 5, it must have received at least $2f + 1$ $(complete, -)$ messages, of which at least $f+1$ must be fault-free.

        \item Therefore, the values sent by the nodes in $A_i$ must be within the set of $(AUX, v)$ messages received by node $i$.

        \item In order for a node to pass Line 5, $values_i$ is the set of values carried by any $|U_i|-f$ messages. %And at time $T$, at least $f + 1$ fault-free messages have been received at every node. 
        At the completion of Line 5, $|U_i| \geq 2f + 1$ because $U_i$ is the set of all nodes which node $i$ has received messages from. By the predicate of Line 5, node $i$ has received at least $2f + 1$ $(complete, -)$ messages. Hence, node $|U_i| \geq 2f + 1$.
        Out of the $|U_i|$ $(AUX, v)$ messages received at node $i$, $f+1$ of these values must be fault-free and seen by every node. $f+1$ of these values must be fault-free because there are at least $2f + 1$ values within $values_i$, at most $f$ of which may be Byzantine, leaving at least $f + 1$ fault-free values. These $f + 1$ values must additionally have been seen by every node within the system because the values in $values_i$ are carried by any $|U_i| - f$ messages, where $|U_i| - f \geq (2f + 1) - f = f + 1$. Thus, all other nodes have seen at least $f + 1$ of the values in $values_i$. Hence, node $i$ and node $j$ must receive a common $(AUX, v)$ message. 
        
        %\item Furthermore, if there is a single element in $C_i[p]$, we know that this value was carried by $|U_i|-f$ nodes, and that this value must be seen by all other nodes. 
        
        \item $j$ completes Line 5 at or after $T_i$; hence, it must receive at least $f+1$ $(AUX, v)$ from the fault-free nodes in $A_i$ %because we know at least $2f +1$ nodes have had their value received by all other nodes by time $T$, 
        %Therefore, $f+1$ of these values must be fault-free and seen by every node. 
        By assumption, each message from a mac-broadcast completed before time $T_i$ must be received by $j$ -- due to the remark 1 in DISC, $j$ has to process them at Line 5.

        \item By Line 7, $v$ must be in $C_j[p]$. 

        \item If there is only one value in $C_j[p]$, then this value must be the value only value in $C_i[p]$. Therefore, $C_j[p] = \{v\} = \{u\}$. 

        \begin{proof}
            Suppose $C_j[p] = \{v\}$ and $C_i[p] = \{u\}$, where $\{v\} \neq \{u\}$. We derive a contradiction.

            Since $C_j[p] = \{v\}$, the only value which appears at least $f + 1$ times in $R_j[p]$ must be $v$. Therefore, $R_j[p]$ has at least $f + 1$ $v$'s and at most $f$ $u$'s.

            Analogously, since $C_i[p] = \{u\}$, the only value which appears at least $f + 1$ times in $R_i[p]$ must be $u$. Therefore, $R_i[p]$ has at least $f + 1$ $u$'s and at most $f$ $v$'s.

            In this scenario, $values_j$ has at least $f + 1$ $v$'s and at most $f$ $u$'s, while $values_i$ has at most $f$ $v$'s and at least $f + 1$ $u$'s.

            All fault-free values which $j$ sees must have been seen by $i$ because because node $j$ completes Line 5 at or after $T_i$. However, node $j$ has at most $f$ $u$'s, but node $i$ must have at least $f + 1$ $u$'s. %Even if $f$ of the $u$'s received by node $i$ are sent from Byzantine nodes, 
            We know that all other nodes have seen at least $f + 1$ of the values in $values_i$. So, $j$ must have seen at least $1$ $u$ from $i$ ... but we need this to be $f +1$ $u$'s to arrive at our contradiction.
            

            %$C_i[p] \subseteq C_j[p]$ because node $j$ completes Line 5 at or after $T_i$. In the time interval from $T_i$ to $T_j$, node $j$ can receive additional $(complete, -)$ messages corresponding to additional $(AUX, v)$ messages whose $v$ fields are added to $R_i[p]$. In this case, $C_i \subset C_j$. Otherwise, $C_i = C_j$.  

            

            
        \end{proof}
    \end{itemize}
    %To do so, we want to make sure that node i and node j will receive a common message of AUX. This seems to hold, because 2f+1 sent a COMPLETE message, and at least f+1 of them are correct. These correct nodes have completed Line 4 -- which means for any other node x at least 1 of them will have its value v considered by x. 
    % 
    % 
\end{proof}

%%%%%

\begin{comment}
    
\begin{algorithm}
\caption{MAC-BRC: Steps at each node $i$}
\label{alg:MAC-BRC}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:}]
    
    \item[] $p_i$ \COMMENT{phase, initialized to $0$}
    
    \item[] $v_i$ \COMMENT{state, initialized to $x_i$, the input at node $i$}

    \item[] $U_i$ \COMMENT{count, initialized to $3f+1$, count of all the nodes that node $i$ knows so far} 

    \item[] $F_i$ \COMMENT{output, initialized to $null$, the output at node $i$}

    \hrulefill
    \begin{multicols}{2}    

    \WHILE{true}
        \STATE $p_i \leftarrow p_i + 1$
        \STATE \textbf{mac-broadcast}$(value, i, v_i, p_i, U_i)$
        %\STATE \textbf{mac-broadcast}$(complete, i)$
        \STATE \textbf{wait until} node $i$ has received \\\hspace{18pt} $\geq U_i - f$ $(complete, -)$ messages
        \STATE $R_i[p_i] \leftarrow$ $v$ field in all received $(value)$ messages \COMMENT{$R_i$ is a multi-set}
        \STATE $U_i \gets |R_i|$
        \STATE $C_i[p_i] \gets$ any value $v$ that appears at least \\\hspace{18pt} $f+1$ times in $R_i[p_i]$
        \STATE $c \gets coinflip()$
        \IF{$C_i[p_i] = \{v\}$}
            \IF{$v = c$}
                \STATE \textbf{mac-broadcast}$(decide, i, v_i, p_i, U_i)$
            \ENDIF
            \STATE $v_i \gets v$
        \ELSE
            \STATE $v_i \gets c$     
        \ENDIF
    \ENDWHILE
    \columnbreak
    \STATE //\textit{Background message handler 1}
    \STATE \textbf{Upon} receive($(decide, j, v, p, U)$) do
    \STATE $D \gets D \cup (j, v, U)$
    \IF{$D$ contains $\geq U_i - f$ unique entries with $(v, U)$ such that $(v = v_i, U \geq U_i - f)$} % To account for Byzantine behavior - assuming Byzantine nodes cannot lie about their identity?
        \IF{$U = U_i$}
            \IF{$v = v_i$} 
                \STATE \textbf{mac-broadcast}($(decide2, i, v_i, p_i, U_i)$) 
            \ELSE % $v \neq v_i$    
                \STATE $v_i \gets c$
                \STATE \textbf{mac-broadcast}($(decide2, i, v_i, p_i, U_i)$)
            \ENDIF
        \ENDIF
        \IF{$U > U_i$}
            \IF{$v = v_i$} 
            \STATE $U_i \gets U$
                \STATE \textbf{mac-broadcast}($(decide2, i, v_i, p_i, U)$) 
            \ELSE % $v \neq v_i$ 
                \STATE \textbf{mac-broadcast}($(decide2, i, v, p_i, U)$)
            \ENDIF
        \ENDIF
        \IF{$U < U_i$}
            \IF{$v = v_i$}
                \STATE \textbf{mac-broadcast}($(decide2, i, v_i, p_i, U_i)$) 
            \ELSE % $v \neq v_i$ 
                \STATE \textbf{mac-broadcast}($(decide2, i, v_i, p_i, U_i)$) 
            \ENDIF
        \ENDIF
    \ENDIF
    
    \hfill
    \STATE //\textit{Background message handler 2}
    \STATE \textbf{Upon} receive($(decide2, j, v, p, U)$) do
    \IF{node $i$ received $(decide2, j, v, p , U)$ from $U_i$ different nodes}
        \STATE $F_i = v_i$
    \ENDIF



\end{multicols}  
\end{algorithmic}
\end{algorithm}

\end{comment}

==> storeCollect.tex <==
\section{Byzantine-Tolerant Consensus with Store-Collect and PKI}
In this section, we implement a Byzantine-tolerant Store-Collect object using PKI.

\subsection{Store-Collect Object}

We employ the construction of the Store-Collect object which is defined in \cite{10.1145/3519270.3538462}. 

\subsection{Public Key Infrastructure (PKI)}

Public Key Infrastructure (PKI) serves as a means by which nodes can sign the messages that they send to other nodes. PKI encompasses the entire technology which provides this guarantee of message authentication and proof of identity via signatures. PKI's have applications to consensus algorithms, specifically for blockchain protocols as in \cite{garay2018bootstrapping}, and are used as an important component of Internet of Things (IoT) systems.

\subsection{Byzantine-Tolerant Consensus with Store-Collect and PKI}

We now consider the case when each node is equipped with PKI. That is, each node can sign the message, and no one can forge it. In this case consensus is possible by building a Store-Collect object.

Including PKI within the context of consensus algorithms, we can allow nodes to sign the messages they send. This way, messages cannot be forged, and Byzantine nodes cannot pretend that they have received messages from other nodes which they have not in fact received. So, we can implement an Byzantine-tolerating store-collect using PKI.

\subsection{Byzantine-Tolerant Store-Collect Object Using PKI}

In the following algorithm, BSC, which implements the a Byzantine-tolerant Store-Collect object using PKI, each $view_i$ within a node's $currentView_i$ is guaranteed to provide authentication that the $view_i$ is indeed signed and sent by node $i$. As in \cite{abraham2022brief}, we denote a message $m$ signed by node $i$ by $\langle m \rangle_i$. We only assume a message is valid if it is properly signed by the sender node. The following algorithm ensures that all nodes within the system agree on the same view of messages even in the presence of Byzantine faults.

Below, $view(v, i, x)$ denotes the $x$-th value received by a correct node, where each node’s $x$-th value is the same for every correct node by Lemma \ref{lemma:x}.

%\lewis{See https://arxiv.org/pdf/2102.07932.pdf 

%and use their notation for signed messages -- you need it for the proof.}

\begin{algorithm}
\caption{BSC Steps at each node $i$}
\label{alg:BEC-SC}
\begin{algorithmic} [1]
\footnotesize
\item[{\bf Local Variables:}]

    %\item[] $R_i$ \COMMENT{$R_i$, initialized to $\emptyset$, contains $v_i$ from each received view} 
    \item[] $view_i$ \COMMENT{view, initialized to $\emptyset$}

    \hrulefill
    
    \item[\textbf{When $Store_i{(v)}$ is invoked}:]
    \STATE $currentView_i \gets view_i \cup \{(v, i)\}$
    \STATE \texttt{mac-broadcast}($Store$, $currentView_i$)
    \STATE \textbf{return} ACK \COMMENT{$Store$ is completed}

    \vspace{3pt}

    \item[\textbf{When $Collect_i$ is invoked}:]
    \STATE $currentView \leftarrow view_i$
    \STATE \texttt{mac-broadcast}($Store$, $currentView$)
    \STATE \textbf{return} $currentView$
    
    \vspace{3pt}
    
    \item[$\slash\slash$ \textit{Background message handler}] %\lewis{I don't think this is working, especially for a Byzantine sender $k$, it's possible that node $i$ has $k$'s value, but none of the other nodes will have $k$'s value.}

    \item[\textbf{Upon} receive($Store$, $view$) \textbf{do}] 
        %\FOR{each $j \in view$}
        %    \STATE $R_j \leftarrow v_j \in view$
        %\ENDFOR
        %\IF{$|R_j| \geq f + 1$ for each $R_j$}
        \FOR{each $j \in view$}
            \IF{$view_i(v, j, x) \neq view(v, j, x)$} 
                \STATE $view \gets view \setminus view(v, j, x)$
            \ENDIF
        \ENDFOR
        \STATE $view_i \gets view_i \cup view$ 
        
        

\end{algorithmic} 
\end{algorithm}

%(v, i, x)
%= i’s x-th value is v
%Which is each element in the view
%That’s something you need to prove

\subsection{Definitions for Store-Collect Object}

We adopt the following definitions and notation from \cite{10.1145/3519270.3538462}.

\begin{definition} [Store]
    A \textbf{Store} operation, $Store_i(v)$, is an operation at node $i$ which stores $v$ into the Store-Collect object.
\end{definition}

\begin{definition} [Collect]
    A \textbf{Collect} operation, $Collect_i$, is an operation which returns a view the most up-to-date values of each node from the Store-Collect object.     
\end{definition}

\begin{definition} [View]
    A \textbf{view} is the value returned by $Collect_i$. A view consists of tuples of the form $V = (v_j, j)$, where $v_j$ denotes the most recent value of a node, $j$. If $j$ is contained within a view $V$, then $V(j) = v_j$, otherwise, $V(j) = \perp$.
\end{definition}

\begin{definition} [Durable]
    Information is defined to be \textbf{durable} if it is not lost even after a crash fault occurs.
\end{definition}

\begin{definition} [Timely]
    Information is defined to be \textbf{timely} if it satisfies real-time constraint -- timely information can be learned from other nodes by contacting a quorum of nodes.
\end{definition}

\begin{definition} [History]
    The \textbf{history} of a Store-Collect object is the partially-ordered set of the executions of Store and Collect operations, including both their invocation (inv) and response (resp) events. A history is denoted $(H, <_H)$, where the set $H$ contains the invocations and responses of Store and Collect operations, and $<_H$ represents the real-time ordering of events in $H$.  
\end{definition}

\begin{definition} {Operation}
    An \textbf{operation} is either a complete execution (invocation and response) of a call to Store, or a complete execution (invocation and response) of a call to Collect. An operation $op_1$ precedes another operation $op_2$ in execution history if $resp(op_1) <_H inv(op_2)$, that is, the response of $op_1$ occurs before the invocation of $op_2$.
\end{definition}

\begin{definition} [Event]
    An \textbf{event} is an invocation or response of a Store or Collect operation. In the execution timeline, if event $e_1$ is occurs before event $e_2$ (an operation $op_1$ is invoked before the invocation of operation $op_2$, this is denoted $e_1 <_H e_2$.
\end{definition}

\begin{definition} [Regularity]
    \textbf{Regularity} is a condition defined on the history, $h$, of a Store-Collect object such that:
    \begin{itemize}
        \item Every Collect $c \in h$ returning $V(j)$ for each node $j$ follows one of two cases:
            \begin{itemize}
                \item [(1)] If $V(j) = v$, then (i) $inv(Store_j(v)) <_H resp(c)$, (ii) there does not exist a $Store_j(v')$ such that $v' \neq v$, and (iii) $resp(Store(v)) <_H resp(Store(j')) <_H inv(c)$.
                \item [(2)] If $v(j) = \perp$, then there does not exist a $Store_j(v) <_H c \in h$.
            \end{itemize}
        \item For any two collects, $c_1$ and $c_2 \in h$ which return views $V_1$ and $V_2$, respectively, if $c_1 <_H c_2$, then $V_1 \preceq V_2$. 
    \end{itemize}
\end{definition}

\begin{definition} [Store-Collect Object]
    An algorithm correctly implements a \textbf{Store-Collect} object if the algorithm's history always satisfies regularity.
\end{definition}

\subsection{Proof of BSC}

By the definition of a Store-Collect object in \cite{10.1145/3519270.3538462}, an algorithm correctly implements the Store-Collect object if every execution of the algorithm results in a history that satisfies regularity. Furthermore, to achieve regularity, all stored messages must be both durable and timely, as defined above.

%\begin{lemma}
%\label{lemma:v-j}
%    A node $i$ can only add a view $v_j$ to $V_i$ if $v_j$ has been sent by a fault-free node. 
%\end{lemma}

%\begin{proof}
%    Upon receiving a $(Store, view)$, a node will add each of the views for every node $j$ to the corresponding set $R_j$ for that node's set of received views at other nodes. There are at most $f$ Byzantine nodes, so if $|R_j| \geq f + 1$, we know that $view$ must have been sent by at least one fault-free node, and is therefore a valid view. Moreover, these messages are signed, so we can be sure that the identity of the sender is truthful. This condition is validated on Line $10$ for each node $j$ in $view$ in order for a $view$ to be added to $view_i$. Therefore, we guarantee that only fault-free values are stored to a node's view.
%\end{proof}

%\begin{lemma}
%\label{lemma:view}
%    If a fault-free node $i$ stores $v$ in its most up-to-date view $V_i$, then all other nodes, including Byzantine nodes, must store $v$ to their current views, $V$.
%\end{lemma}

%\begin{proof}
%    If a fault-free node $i$ stores $v$ in its current view, $V_i$, we know that node $i$ must have sent the mac-broadcast $Store_i(v)$ and received the corresponding ACK for this mac-broadcast. A node $i$ will execute a $Store$ operation upon receiving a signed message $\langle v\rangle_j$. We know that every node will have received $(Store, currentView_i)$ once the mac-broadcast completes and the ACK is returned on Line $3$, and will subsequently update their $currentView$ to reflect this new information. Moreover, a Byzantine node cannot fake the values sent by other nodes because each message is signed by the sender node.
%\end{proof}

%\begin{lemma}
%\label{lemma:collect}
%    Calls to $Collect_i$ will return up-to-date views.
%\end{lemma}

%\begin{proof}
%    By Lemma \ref{lemma:view}, we know that the views added to a node's $currentView$ must be seen by all other nodes as well, so they will be in the views of other nodes. Therefore, all $currentView$'s returned by invocations of $Collect_i$ must contain the same values as all nodes. 
%\end{proof}

\begin{lemma}
\label{lemma:x}
    The $x$-th value in a view at every node is the same for every correct node, where $x$ is the sequence number of each value $v$ in node $i$'s view.
    %That is each node’s x-th value should be the same for every correct node
\end{lemma}

\begin{proof}
%I understand, so if we have nodes A and B and  values X1 and X2 received by both nodes from sender X: then if node A said that value X1 was newer, and node B said that X2 was newer, then we know that X is Byzantine. However, node A can have both X1 and X2 without thinking X is Byzantine, it will just update its view to have the newer value (as long as this aligns with what B sees as well).    
    Every correct node will track the sequence number of the value $v$ received from all other nodes. That is, if node $i$ has received $x$ values from node $j$, then the sequence number for node $j$'s value in $view_i$ will be $x$. We denote this value as $view_i(v, j, x)$. Every correct node updates its view upon receiving a message of the form $(Store, view)$ by adding the values of each node in the view to $view_i$ if the sequence number for each of the respective values from other nodes match. If values $v_1$ and $v_2$ from the same node $b$ have equal sequence numbers $x$ (if $view(v_1, j, x) \neq view(v_2, j, x)$ for a specific $j$ and $x$), then node $b$ must be Byzantine, and the incoming value $v_2$ will not both be added to $i$'s view. Additionally, all nodes see the views of all other nodes who  invoke $Store(v)$ for incoming values due to the mac-broadcast. Each time a node broadcasts its view, it increments the sequence number for the values of this view. Therefore, all values which are in any correct node's view must agree in value and sequence number to all other nodes which have received this value. 
\end{proof}

\begin{lemma}
\label{lemma:byz}
    If a Byzantine node sends differing values to two nodes $i$ and $j$, then these values will be disregarded.
\end{lemma}

\begin{proof}
     Consider two nodes, node $i$ and node $j$, which each receive a value $v_b$ from a Byzantine node $b$. Node $i$ sees all of the values within the views sent by $j$, and node $j$ sees all of the values within the views sent by $i$. Therefore, if nodes $i$ and $j$ receive different values from $b$, they will be able to identify that node $b$ is Byzantine, and will hence disregard the values $(v_b, b)$ within their respective views by removing it from the set at Line $9$. 
\end{proof}

\begin{lemma}
\label{lemma:id-byz}
    If any node identifies a node $b$ to be Byzantine, then all other nodes will learn this information as well.
\end{lemma}

\begin{proof}
    By Lemma \ref{lemma:byz}, Byzantine values will be identified and disregarded. Due to the PKI, all messages are signed by the sender. Therefore, upon receiving differing messages from the same node, the receiving node, will be able to identify the sender of these values as a Byzantine node. Subsequently, all other nodes will identify $b$ as a Byzantine node and disregard all future values from $b$. At all nodes $i$:
    \begin{itemize}
        \item Node $i$ will receive contradictory values and disregard them as Byzantine by Lemma \ref{lemma:byz}, so node $i$ will learn that $b$ is Byzantine and disregard all future values as well.
        \item Another fault-free node $j$ will identify node $b$ as a Byzantine node, and broadcast this information to all other nodes, so node $i$ will learn that node $b$ is Byzantine.
    \end{itemize}

    Therefore, after one node discovers a Byzantine node $b$, all other nodes will learn this information and disregard the values signed by $b$.
\end{proof}

\begin{theorem}
    BSC implements a Store-Collect object with Byzantine faults and the use of PKI.
\end{theorem}

\begin{proof}

    Our proof of the Store-Collect object is the same for Byzantine faults as it is for crash faults because Byzantine nodes will be identified for sending mismatch values and its values will be disregarded by fault-free nodes. 

    For each node $j$, a $Collect_i$ operation, $c$, can return $V$ such that (i) $V(j) = \perp$, or (ii) $V(j) = v$.

    \begin{itemize}
        \item [(i)] $V(j) = v$: $inv(Store_j(v)) <_H resp(c)$, so we know that $v \in V(j)$. And, there is no other $Store_j(v')$ which completes between $inv(Store_j(v))$ and $inv(c)$.

        \item [(ii)] $V(j) = \perp$: There is no $Store_j(v) <_H c$ since node $i$ has not received any message from $j$'s mac-broadcast. Hence, either (i) $j$'s mac-broadcast has not completed, or (ii) node $j$ has not invoked a mac-broadcast.
    \end{itemize}

    Furthermore, we know that $V_1 \preceq V_2$ because when node $i$ receives an ACK from its mac-broadcast, all of the fault-free nodes must have received $i$'s message. Thus, if collects $c_1 <_H c_2$, returning $V_1$ and $V_2$, respectively, we know that $V_1 \preceq V_2$.

    If a node $i$ adds $V(j) = v$ to $view_i$, then $v$ must be fault-free, otherwise, it would be discarded as Byzantine by Lemma \ref{lemma:byz}. Moreover, by Lemma \ref{lemma:x}, for any two views $V_i$ and $V_j$ as above, all values $v \in V_i, V_j$ with the same identity and sequence number will be equal. Byzantine nodes cannot cause conflicting views because as we have demonstrated, Byzantine values will be discarded. Moreover, by Lemma \ref{lemma:id-byz}, upon identification of a Byzantine node within the system, all nodes will learn this information and will disregard any subsequent values from $b$, so $V_i$ and $V_j$ will remain consistent despite the presence of Byzantine faults.
    

    
    
\end{proof}


